AgileCoder: Dynamic Collaborative Agents for Software Development based on Agile Methodology

Software agents have emerged as promising tools for addressing complex software engineering tasks. Existing works, on the other hand, frequently oversimplify software development workflows, despite the fact that such workflows are typically more complex in the real world. Thus, we propose AgileCoder, a multi agent system that integrates Agile Methodology (AM) into the framework. This system assigns specific AM roles - such as Product Manager, Developer, and Tester to different agents, who then collaboratively develop software based on user inputs. AgileCoder enhances development efficiency by organizing work into sprints, focusing on incrementally developing software through sprints. Additionally, we introduce Dynamic Code Graph Generator, a module that creates a Code Dependency Graph dynamically as updates are made to the codebase. This allows agents to better comprehend the codebase, leading to more precise code generation and modifications throughout the software development process. AgileCoder surpasses existing benchmarks, like ChatDev and MetaGPT, establishing a new standard and showcasing the capabilities of multi agent systems in advanced software engineering environments.

==> latex/workflow.tex <==
% \methodname is a progressive development programming framework for LLMs-based multi-agent collaboration systems. The overview is shown in Figure \ref{fig:overview-agilecoder}. Our main concept is inspired by Agile Scrum methodology in software development, which allows incremental development and facilitates communication among agents to rectify the errors at the previous stages.


% \subsection{Incremental development}
% \citet{zhou2023leasttomost, khot2023decomposed} shows that LLMs can solve a complex problem by decomposing it into smaller and manageable subtasks and a final solution is merged from those of the subtasks. In the context of the software development, a software is usually non-trivial, so it is hard for an LLM based-agent to complete without any error. Instead, the collaboration of multiple agents with diverse skills can leverage fully a wide range of expertise of agents as well as enhance the specialization with each engaging in specific phases to make the task-solving process easier. There are some existing work \citep{qian2023chatdev, hong2024metagpt} that propose multi-agent communicative frameworks for programming tasks. ChatDev \citep{qian2023chatdev} breaks down a task into sequential subtasks, which mirrors the established waterfall model; meanwhile, MetaGPT \citep{hong2024metagpt} incorporates Standardized Operating Procedures into prompts and it also employs the waterfall model to manage subtasks. Although the waterfall model exhibits the effectiveness in ChatDev \citep{qian2023chatdev} and MetaGPT \citep{hong2024metagpt}, it is currently no longer popular in practice and replaced by Agile Scrum methodology. Agile Scrum methodology offers some advantages over the waterfall model such as higher-quality and course-correction.  Because of the feedback after each sprint, Scrum allows to accommodate changes and modify features. In the early stages, there may be infeasible subtasks in the plan or existing bugs that are not fixed, which can be rectified in the later sprints. Moreover, tasks in Scrum are prioritized by order of importance, meaning first completed tasks lay the foundation for further sprints. This makes the development process easier to achieve the goal.

\section{Communication Mechanism Among Agents}
In \methodnamews, we use a dual-agent conversation design for all the phases since they can be modeled to involve only two agents, thereby avoiding complex multi-agent
topologies and effectively streamlining the agreement process. In particular, one agent serves as an instructor and the other plays an assistant, and both interact with each other in order to solve specific goals. The instructor provides instructions and directs the conversation towards task completion, and the assistant follows the guidance and uses the knowledge and skills to accomplish the task. They may experience multiple turns until they reach a consensus.

To maintain consistency between previous and upcoming messages in a dialogue, we use a mechanism called Message Stream $\mathbf{S}$ to keep all emitted messages, so $\mathbf{S}$ serves as a working memory for agents to make responses seamlessly continuous. Formally, let $i_t$ and $a_t$ be the message produced by the instructor and the assistant in the time step $t$, respectively, so $\mathbf{S}_t$ is

$$
\mathbf{S}_t = [(i_1, a_1), (i_2, a_2), ..., (i_t, a_t)]
$$
In the subsequent time step $t+1$, the instructor will consider the historical dialogue $S_t$; specifically, the instructor will determine whether $a_t$ satisfies the instructions and then give the next guidance $t_{t+1}$. Meanwhile, the assistant receives $\mathbf{S}_t$ and the new instruction $i_{t+1}$ to generate an appropriate answer $a_{t+1}$. If $a_{t+1}$ meets the predefined termination criteria or $t + 1$ exceeds the maximum number of turns, the conversation will come to an end, and we will store the message $a_{t+1}$ in the environment for following conversations. We just need to retain the $a_{t+1}$ as it is the complete answer for the original instruction, ensuring that only relevant and useful information is saved.
% \subsection{Scrum workflow among agents}
% To make agents interact with each other effectively, we need to establish a workflow. In AgileCoder, we adapt Agile Scrum methodology in software development, which enables the collaboration among agents through multiple sprints. Therefore, after each sprint, we obtain its outputs and determine whether they meet the sprint's requirements to have useful feedback for next sprints, akin to the interactive and incremental development. The progressive development can ensure the quality of products as in a certain sprint, all efforts are concentrated on some subtasks, and issues existing from previous sprints can be fixed in subsequent sprints by adjusting the goals and requirements.
\subsection{Communication Protocol}
Following previous works \citep{qian2023chatdev}, we utilize unconstrained natural language as a communication interface. Using the natural language prompts offers a high degree of versatility, so we can easily modify prompts without nearly influencing the entire system, such as adding new constraints for outputs or changing the output format. 

Furthermore, to enhance the quality and likelihood of task completion, \methodname employs prompt engineering that only takes place once at the start of each conversation, which helps agents understand requirements and goals of tasks that are associated with the dialogue, so they can generate appropriate responses towards completing tasks. When a conversation is initiated, the instructor and the assistant will interact with each other autonomously until a consensus is reached without human intervention.

\subsection{Global Message Pool}
To make the information flow seamlessly from the start to the end, we use a global sharing environment that stores the outputs of all the conversations. Additionally, the sharing environment also records the entire process, such as done/undone/failed works, which provides useful context for agents to make the right decisions. Consequently, the amount of information stored in the environment can be large, which may be ineffective if providing all data to agents. Therefore, each conversation in \methodname registers the global message pool to seek relevant data to assist in solving the task. For instance, when writing a sprint backlog, the Product Owner just needs to know product backlog, complete and unsolved tasks, and may ignore source code. Meanwhile, when patching a bug, the Programmer only knows the location of buggy code and relevant code, but the product backlog. This message pool helps to not only avoid the overwhelming issue for agents when they receive too much information but also ensure that agents have access to a unifying and latest source of information.



% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{images/overview.png}
%     \caption{An overview of \methodnamews}
%     \label{fig:overview-agilecoder}
% \end{figure*}


% \begin{table}
% \centering
% \resizebox{0.5\textwidth}{!}{
% \begin{tabular}{l|ccc} 
% \hline
% \textbf{Framework Capabiliy} & \textbf{ChatDev}             & \textbf{MetaGPT}             & \textbf{AgileCoder}           \\ 
% \hline
% API interface generation     & \textcolor{red}{\ding{55}}   & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}}  \\
% Code generation              & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}}  \\
% Role-based task management   & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}}  \\
% Code review                  & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}}  \\
% Flexible target              & \textcolor{red}{\ding{55}}   & \textcolor{red}{\ding{55}}   & \textcolor{green}{\ding{51}}  \\
% Incremental developments     & \textcolor{red}{\ding{55}}   & \textcolor{red}{\ding{55}}   & \textcolor{green}{\ding{51}}  \\
% \hline
% \end{tabular}}
% \caption{Compare with other Multi-agent frameworks}
% \label{compareing}
% \end{table}
